Impact of Hole-ice Calibration on High Energy Event Reconstruction with the IceCube Upgrade

The IceCube Upgrade, currently under construction at the geographic South Pole, is the next development stage of the IceCube detector. It will consist of seven new columns of novel optical sensors and advanced calibration devices densely deployed at the centre of the existing array. The sensors are frozen into the ice in boreholes created by hot water drilling. The refreezing forms hole ice around modules with optical properties that differ from the surrounding glacial ice. A key objective of the IceCube Upgrade is to enhance our understanding of the optical properties of both bulk ice and refrozen hole ice. Precise ice modelling is crucial for the directional reconstruction of TeV-PeV neutrinos, as resolutions at such high energies can be strongly impacted by uncertainties in ice properties and optical sensor response. An improved directional reconstruction performance will translate to a boost in neutrino source sensitivities using IceCube data collected over the last 12 years. In this contribution, we present the expected improvements in reconstruction performance resulting from advances in hole-ice modelling and the resulting impact on IceCube's sensitivity to astrophysical neutrino sources across three distinct event samples.

==> authorlist_IC_Gen2.tex <==
\section*{Full Author List: IceCube-Gen2 Collaboration (May 17, 2025)}

\scriptsize
\noindent
R. Abbasi$^{16}$,
M. Ackermann$^{77}$,
J. Adams$^{21}$,
S. K. Agarwalla$^{46,\: 78}$,
J. A. Aguilar$^{10}$,
M. Ahlers$^{25}$,
J.M. Alameddine$^{26}$,
N. M. Amin$^{52}$,
K. Andeen$^{49}$,
G. Anton$^{29}$,
C. Arg{\"u}elles$^{13}$,
Y. Ashida$^{63}$,
S. Athanasiadou$^{77}$,
J. Audehm$^{1}$,
S. N. Axani$^{52}$,
R. Babu$^{27}$,
X. Bai$^{60}$,
A. Balagopal V.$^{46}$,
M. Baricevic$^{46}$,
S. W. Barwick$^{33}$,
V. Basu$^{63}$,
R. Bay$^{6}$,
J. Becker Tjus$^{9,\: 79}$,
P. Behrens$^{1}$,
J. Beise$^{75}$,
C. Bellenghi$^{30}$,
B. Benkel$^{77}$,
S. BenZvi$^{62}$,
D. Berley$^{22}$,
E. Bernardini$^{58,\: 80}$,
D. Z. Besson$^{39}$,
A. Bishop$^{46}$,
E. Blaufuss$^{22}$,
L. Bloom$^{71}$,
S. Blot$^{77}$,
M. Bohmer$^{30}$,
F. Bontempo$^{34}$,
J. Y. Book Motzkin$^{13}$,
J. Borowka$^{1}$,
C. Boscolo Meneguolo$^{58,\: 80}$,
S. B{\"o}ser$^{47}$,
O. Botner$^{75}$,
J. B{\"o}ttcher$^{1}$,
S. Bouma$^{29}$,
J. Braun$^{46}$,
B. Brinson$^{4}$,
Z. Brisson-Tsavoussis$^{36}$,
R. T. Burley$^{2}$,
M. Bustamante$^{25}$,
D. Butterfield$^{46}$,
M. A. Campana$^{59}$,
K. Carloni$^{13}$,
M. Cataldo$^{29}$,
S. Chattopadhyay$^{46,\: 78}$,
N. Chau$^{10}$,
Z. Chen$^{66}$,
D. Chirkin$^{46}$,
B. A. Clark$^{22}$,
R. Clark$^{41}$,
A. Coleman$^{75}$,
P. Coleman$^{1}$,
G. H. Collin$^{14}$,
J. M. Conrad$^{14}$,
R. Corley$^{63}$,
D. F. Cowen$^{72,\: 73}$,
B. Dasgupta$^{50}$,
C. Deaconu$^{17,\: 20}$,
C. De Clercq$^{11}$,
S. De Kockere$^{11}$,
J. J. DeLaunay$^{72}$,
D. Delgado$^{13}$,
S. Deng$^{1}$,
A. Desai$^{46}$,
P. Desiati$^{46}$,
K. D. de Vries$^{11}$,
G. de Wasseige$^{43}$,
J. C. D{\'\i}az-V{\'e}lez$^{46}$,
S. DiKerby$^{27}$,
M. Dittmer$^{51}$,
G. Do$^{1}$,
A. Domi$^{29}$,
L. Draper$^{63}$,
L. Dueser$^{1}$,
H. Dujmovic$^{46}$,
D. Durnford$^{28}$,
K. Dutta$^{47}$,
M. A. DuVernois$^{46}$,
T. Egby$^{5}$,
T. Ehrhardt$^{47}$,
L. Eidenschink$^{30}$,
A. Eimer$^{29}$,
P. Eller$^{30}$,
E. Ellinger$^{76}$,
D. Els{\"a}sser$^{26}$,
R. Engel$^{34,\: 35}$,
H. Erpenbeck$^{46}$,
W. Esmail$^{51}$,
J. Evans$^{22}$,
J. J. Evans$^{48}$,
P. A. Evenson$^{52}$,
K. L. Fan$^{22}$,
K. Fang$^{46}$,
K. Farrag$^{15}$,
A. R. Fazely$^{5}$,
A. Fedynitch$^{69}$,
N. Feigl$^{8}$,
C. Finley$^{65}$,
L. Fischer$^{77}$,
B. Flaggs$^{52}$,
D. Fox$^{72}$,
A. Franckowiak$^{9}$,
T. Fujii$^{56}$,
S. Fukami$^{77}$,
P. F{\"u}rst$^{1}$,
J. Gallagher$^{45}$,
E. Ganster$^{1}$,
A. Garcia$^{13}$,
G. Garg$^{46,\: 78}$,
E. Genton$^{13}$,
L. Gerhardt$^{7}$,
A. Ghadimi$^{71}$,
P. Giri$^{40}$,
C. Glaser$^{75}$,
T. Gl{\"u}senkamp$^{75}$,
S. Goswami$^{37,\: 38}$,
A. Granados$^{27}$,
D. Grant$^{12}$,
S. J. Gray$^{22}$,
S. Griffin$^{46}$,
S. Griswold$^{62}$,
D. Guevel$^{46}$,
C. G{\"u}nther$^{1}$,
P. Gutjahr$^{26}$,
C. Ha$^{64}$,
C. Haack$^{29}$,
A. Hallgren$^{75}$,
S. Hallmann$^{77}$,
L. Halve$^{1}$,
F. Halzen$^{46}$,
L. Hamacher$^{1}$,
M. Ha Minh$^{30}$,
M. Handt$^{1}$,
K. Hanson$^{46}$,
J. Hardin$^{14}$,
A. A. Harnisch$^{27}$,
P. Hatch$^{36}$,
A. Haungs$^{34}$,
J. H{\"a}u{\ss}ler$^{1}$,
D. Heinen$^{1}$,
K. Helbing$^{76}$,
J. Hellrung$^{9}$,
B. Hendricks$^{73,\: 74}$,
L. Hennig$^{29}$,
J. Henrichs$^{77}$,
L. Heuermann$^{1}$,
N. Heyer$^{75}$,
S. Hickford$^{76}$,
A. Hidvegi$^{65}$,
C. Hill$^{15}$,
G. C. Hill$^{2}$,
K. D. Hoffman$^{22}$,
B. Hoffmann$^{34}$,
S. Hori$^{46}$,
K. Hoshina$^{46,\: 81}$,
M. Hostert$^{13}$,
W. Hou$^{34}$,
T. Huber$^{34}$,
T. Huege$^{34}$,
K. Hultqvist$^{65}$,
R. Hussain$^{46}$,
K. Hymon$^{26,\: 69}$,
A. Ishihara$^{15}$,
T. Ishii$^{56}$,
W. Iwakiri$^{15}$,
M. Jacquart$^{46}$,
S. Jain$^{46}$,
O. Janik$^{29}$,
M. Jansson$^{67}$,
M. Jeong$^{63}$,
M. Jin$^{13}$,
O. Kalekin$^{29}$,
N. Kamp$^{13}$,
D. Kang$^{34}$,
W. Kang$^{67}$,
X. Kang$^{59}$,
A. Kappes$^{51}$,
L. Kardum$^{26}$,
T. Karg$^{77}$,
M. Karl$^{30}$,
A. Karle$^{46}$,
A. Katil$^{28}$,
T. Katori$^{41}$,
U. Katz$^{29}$,
M. Kauer$^{46}$,
J. L. Kelley$^{46}$,
M. Khanal$^{63}$,
A. Khatee Zathul$^{46}$,
A. Kheirandish$^{37,\: 38}$,
J. Kiryluk$^{66}$,
M. Kleifges$^{34}$,
C. Klein$^{29}$,
S. R. Klein$^{6,\: 7}$,
T. Kobayashi$^{56}$,
Y. Kobayashi$^{15}$,
A. Kochocki$^{27}$,
H. Kolanoski$^{8}$,
T. Kontrimas$^{30}$,
L. K{\"o}pke$^{47}$,
C. Kopper$^{29}$,
D. J. Koskinen$^{25}$,
P. Koundal$^{52}$,
M. Kowalski$^{8,\: 77}$,
T. Kozynets$^{25}$,
I. Kravchenko$^{40}$,
N. Krieger$^{9}$,
J. Krishnamoorthi$^{46,\: 78}$,
T. Krishnan$^{13}$,
E. Krupczak$^{27}$,
A. Kumar$^{77}$,
E. Kun$^{9}$,
N. Kurahashi$^{59}$,
N. Lad$^{77}$,
M. J. Larson$^{22}$,
F. Lauber$^{76}$,
K. Leonard DeHolton$^{73}$,
A. Leszczy{\'n}ska$^{52}$,
J. Liao$^{4}$,
M. Liu$^{40}$,
M. Liubarska$^{28}$,
M. Lohan$^{50}$,
J. LoSecco$^{55}$,
C. Love$^{59}$,
L. Lu$^{46}$,
F. Lucarelli$^{31}$,
Y. Lyu$^{6,\: 7}$,
J. Madsen$^{46}$,
E. Magnus$^{11}$,
K. B. M. Mahn$^{27}$,
Y. Makino$^{46}$,
E. Manao$^{30}$,
S. Mancina$^{58,\: 82}$,
S. Mandalia$^{42}$,
W. Marie Sainte$^{46}$,
I. C. Mari{\c{s}}$^{10}$,
S. Marka$^{54}$,
Z. Marka$^{54}$,
M. Marsee$^{71}$,
L. Marten$^{1}$,
I. Martinez-Soler$^{13}$,
R. Maruyama$^{53}$,
F. Mayhew$^{27}$,
F. McNally$^{44}$,
J. V. Mead$^{25}$,
K. Meagher$^{46}$,
S. Mechbal$^{77}$,
A. Medina$^{24}$,
M. Meier$^{15}$,
Y. Merckx$^{11}$,
L. Merten$^{9}$,
Z. Meyers$^{77}$,
M. Mikhailova$^{39}$,
A. Millsop$^{41}$,
J. Mitchell$^{5}$,
T. Montaruli$^{31}$,
R. W. Moore$^{28}$,
Y. Morii$^{15}$,
R. Morse$^{46}$,
A. Mosbrugger$^{29}$,
M. Moulai$^{46}$,
D. Mousadi$^{77}$,
T. Mukherjee$^{34}$,
M. Muzio$^{72,\: 73,\: 74}$,
R. Naab$^{77}$,
M. Nakos$^{46}$,
A. Narayan$^{50}$,
U. Naumann$^{76}$,
J. Necker$^{77}$,
A. Nelles$^{29,\: 77}$,
L. Neste$^{65}$,
M. Neumann$^{51}$,
H. Niederhausen$^{27}$,
M. U. Nisa$^{27}$,
K. Noda$^{15}$,
A. Noell$^{1}$,
A. Novikov$^{52}$,
E. Oberla$^{17,\: 20}$,
A. Obertacke Pollmann$^{15}$,
V. O'Dell$^{46}$,
A. Olivas$^{22}$,
R. Orsoe$^{30}$,
J. Osborn$^{46}$,
E. O'Sullivan$^{75}$,
V. Palusova$^{47}$,
L. Papp$^{30}$,
A. Parenti$^{10}$,
N. Park$^{36}$,
E. N. Paudel$^{71}$,
L. Paul$^{60}$,
C. P{\'e}rez de los Heros$^{75}$,
T. Pernice$^{77}$,
T. C. Petersen$^{25}$,
J. Peterson$^{46}$,
A. Pizzuto$^{46}$,
M. Plum$^{60}$,
A. Pont{\'e}n$^{75}$,
Y. Popovych$^{47}$,
M. Prado Rodriguez$^{46}$,
B. Pries$^{27}$,
R. Procter-Murphy$^{22}$,
G. T. Przybylski$^{7}$,
L. Pyras$^{63}$,
J. Rack-Helleis$^{47}$,
N. Rad$^{77}$,
M. Rameez$^{50}$,
M. Ravn$^{75}$,
K. Rawlins$^{3}$,
Z. Rechav$^{46}$,
A. Rehman$^{52}$,
E. Resconi$^{30}$,
S. Reusch$^{77}$,
C. D. Rho$^{67}$,
W. Rhode$^{26}$,
B. Riedel$^{46}$,
M. Riegel$^{34}$,
A. Rifaie$^{76}$,
E. J. Roberts$^{2}$,
S. Robertson$^{6,\: 7}$,
S. Rodan$^{67,\: 68}$,
M. Rongen$^{29}$,
C. Rott$^{63}$,
T. Ruhe$^{26}$,
L. Ruohan$^{30}$,
D. Ryckbosch$^{32}$,
I. Safa$^{46}$,
J. Saffer$^{35}$,
D. Salazar-Gallegos$^{27}$,
P. Sampathkumar$^{34}$,
A. Sandrock$^{76}$,
P. Sandstrom$^{46}$,
G. Sanger-Johnson$^{27}$,
M. Santander$^{71}$,
S. Sarkar$^{57}$,
J. Savelberg$^{1}$,
P. Savina$^{46}$,
P. Schaile$^{30}$,
M. Schaufel$^{1}$,
H. Schieler$^{34}$,
S. Schindler$^{29}$,
L. Schlickmann$^{47}$,
B. Schl{\"u}ter$^{51}$,
F. Schl{\"u}ter$^{10}$,
N. Schmeisser$^{76}$,
T. Schmidt$^{22}$,
F. G. Schr{\"o}der$^{34,\: 52}$,
L. Schumacher$^{29}$,
S. Schwirn$^{1}$,
S. Sclafani$^{22}$,
D. Seckel$^{52}$,
M. Seikh$^{39}$,
S. Seunarine$^{61}$,
M. H. Shaevitz$^{54}$,
R. Shah$^{59}$,
S. Shefali$^{35}$,
N. Shimizu$^{15}$,
M. Silva$^{46}$,
B. Skrzypek$^{6}$,
R. Snihur$^{46}$,
J. Soedingrekso$^{26}$,
A. S{\o}gaard$^{25}$,
D. Soldin$^{63}$,
P. Soldin$^{1}$,
G. Sommani$^{9}$,
C. Spannfellner$^{30}$,
G. M. Spiczak$^{61}$,
C. Spiering$^{77}$,
J. Stachurska$^{32}$,
M. Stamatikos$^{24}$,
T. Stanev$^{52}$,
T. Stezelberger$^{7}$,
J. Stoffels$^{11}$,
T. St{\"u}rwald$^{76}$,
T. Stuttard$^{25}$,
G. W. Sullivan$^{22}$,
I. Taboada$^{4}$,
A. Taketa$^{70}$,
H. K. M. Tanaka$^{70}$,
S. Ter-Antonyan$^{5}$,
A. Terliuk$^{30}$,
W. G. Thompson$^{13}$,
J. Thwaites$^{46}$,
S. Tilav$^{52}$,
K. Tollefson$^{27}$,
C. T{\"o}nnis$^{67}$,
J. Torres$^{23,\: 24}$,
S. Toscano$^{10}$,
D. Tosi$^{46}$,
A. Trettin$^{77}$,
Y. Tsunesada$^{56}$,
J. P. Twagirayezu$^{27}$,
M. A. Unland Elorrieta$^{51}$,
A. K. Upadhyay$^{46,\: 78}$,
K. Upshaw$^{5}$,
A. Vaidyanathan$^{49}$,
N. Valtonen-Mattila$^{9,\: 75}$,
J. Vandenbroucke$^{46}$,
T. Van Eeden$^{77}$,
N. van Eijndhoven$^{11}$,
J. van Santen$^{77}$,
J. Vara$^{51}$,
F. Varsi$^{35}$,
D. Veberic$^{34}$,
J. Veitch-Michaelis$^{46}$,
M. Venugopal$^{34}$,
S. Vergara Carrasco$^{21}$,
S. Verpoest$^{52}$,
A. Vieregg$^{17,\: 18,\: 19,\: 20}$,
A. Vijai$^{22}$,
J. Villarreal$^{14}$,
C. Walck$^{65}$,
A. Wang$^{4}$,
D. Washington$^{73}$,
C. Weaver$^{27}$,
P. Weigel$^{14}$,
A. Weindl$^{34}$,
A. Y. Wen$^{13}$,
C. Wendt$^{46}$,
J. Werthebach$^{26}$,
M. Weyrauch$^{34}$,
N. Whitehorn$^{27}$,
C. H. Wiebusch$^{1}$,
D. R. Williams$^{71}$,
S. Wissel$^{72,\: 73,\: 74}$,
L. Witthaus$^{26}$,
M. Wolf$^{30}$,
G. W{\"o}rner$^{34}$,
G. Wrede$^{29}$,
S. Wren$^{48}$,
X. W. Xu$^{5}$,
J. P. Ya{\textbackslash}{\textasciitilde}nez$^{28}$,
E. Yildizci$^{46}$,
S. Yoshida$^{15}$,
R. Young$^{39}$,
F. Yu$^{13}$,
S. Yu$^{63}$,
T. Yuan$^{46}$,
A. Zegarelli$^{9}$,
S. Zhang$^{27}$,
Z. Zhang$^{66}$,
P. Zhelnin$^{13}$,
S. Zierke$^{1}$,
P. Zilberman$^{46}$,
M. Zimmerman$^{46}$
\\
\\
$^{1}$ III. Physikalisches Institut, RWTH Aachen University, D-52056 Aachen, Germany \\
$^{2}$ Department of Physics, University of Adelaide, Adelaide, 5005, Australia \\
$^{3}$ Dept. of Physics and Astronomy, University of Alaska Anchorage, 3211 Providence Dr., Anchorage, AK 99508, USA \\
$^{4}$ School of Physics and Center for Relativistic Astrophysics, Georgia Institute of Technology, Atlanta, GA 30332, USA \\
$^{5}$ Dept. of Physics, Southern University, Baton Rouge, LA 70813, USA \\
$^{6}$ Dept. of Physics, University of California, Berkeley, CA 94720, USA \\
$^{7}$ Lawrence Berkeley National Laboratory, Berkeley, CA 94720, USA \\
$^{8}$ Institut f{\"u}r Physik, Humboldt-Universit{\"a}t zu Berlin, D-12489 Berlin, Germany \\
$^{9}$ Fakult{\"a}t f{\"u}r Physik {\&} Astronomie, Ruhr-Universit{\"a}t Bochum, D-44780 Bochum, Germany \\
$^{10}$ Universit{\'e} Libre de Bruxelles, Science Faculty CP230, B-1050 Brussels, Belgium \\
$^{11}$ Vrije Universiteit Brussel (VUB), Dienst ELEM, B-1050 Brussels, Belgium \\
$^{12}$ Dept. of Physics, Simon Fraser University, Burnaby, BC V5A 1S6, Canada \\
$^{13}$ Department of Physics and Laboratory for Particle Physics and Cosmology, Harvard University, Cambridge, MA 02138, USA \\
$^{14}$ Dept. of Physics, Massachusetts Institute of Technology, Cambridge, MA 02139, USA \\
$^{15}$ Dept. of Physics and The International Center for Hadron Astrophysics, Chiba University, Chiba 263-8522, Japan \\
$^{16}$ Department of Physics, Loyola University Chicago, Chicago, IL 60660, USA \\
$^{17}$ Dept. of Astronomy and Astrophysics, University of Chicago, Chicago, IL 60637, USA \\
$^{18}$ Dept. of Physics, University of Chicago, Chicago, IL 60637, USA \\
$^{19}$ Enrico Fermi Institute, University of Chicago, Chicago, IL 60637, USA \\
$^{20}$ Kavli Institute for Cosmological Physics, University of Chicago, Chicago, IL 60637, USA \\
$^{21}$ Dept. of Physics and Astronomy, University of Canterbury, Private Bag 4800, Christchurch, New Zealand \\
$^{22}$ Dept. of Physics, University of Maryland, College Park, MD 20742, USA \\
$^{23}$ Dept. of Astronomy, Ohio State University, Columbus, OH 43210, USA \\
$^{24}$ Dept. of Physics and Center for Cosmology and Astro-Particle Physics, Ohio State University, Columbus, OH 43210, USA \\
$^{25}$ Niels Bohr Institute, University of Copenhagen, DK-2100 Copenhagen, Denmark \\
$^{26}$ Dept. of Physics, TU Dortmund University, D-44221 Dortmund, Germany \\
$^{27}$ Dept. of Physics and Astronomy, Michigan State University, East Lansing, MI 48824, USA \\
$^{28}$ Dept. of Physics, University of Alberta, Edmonton, Alberta, T6G 2E1, Canada \\
$^{29}$ Erlangen Centre for Astroparticle Physics, Friedrich-Alexander-Universit{\"a}t Erlangen-N{\"u}rnberg, D-91058 Erlangen, Germany \\
$^{30}$ Physik-department, Technische Universit{\"a}t M{\"u}nchen, D-85748 Garching, Germany \\
$^{31}$ D{\'e}partement de physique nucl{\'e}aire et corpusculaire, Universit{\'e} de Gen{\`e}ve, CH-1211 Gen{\`e}ve, Switzerland \\
$^{32}$ Dept. of Physics and Astronomy, University of Gent, B-9000 Gent, Belgium \\
$^{33}$ Dept. of Physics and Astronomy, University of California, Irvine, CA 92697, USA \\
$^{34}$ Karlsruhe Institute of Technology, Institute for Astroparticle Physics, D-76021 Karlsruhe, Germany \\
$^{35}$ Karlsruhe Institute of Technology, Institute of Experimental Particle Physics, D-76021 Karlsruhe, Germany \\
$^{36}$ Dept. of Physics, Engineering Physics, and Astronomy, Queen's University, Kingston, ON K7L 3N6, Canada \\
$^{37}$ Department of Physics {\&} Astronomy, University of Nevada, Las Vegas, NV 89154, USA \\
$^{38}$ Nevada Center for Astrophysics, University of Nevada, Las Vegas, NV 89154, USA \\
$^{39}$ Dept. of Physics and Astronomy, University of Kansas, Lawrence, KS 66045, USA \\
$^{40}$ Dept. of Physics and Astronomy, University of Nebraska{\textendash}Lincoln, Lincoln, Nebraska 68588, USA \\
$^{41}$ Dept. of Physics, King's College London, London WC2R 2LS, United Kingdom \\
$^{42}$ School of Physics and Astronomy, Queen Mary University of London, London E1 4NS, United Kingdom \\
$^{43}$ Centre for Cosmology, Particle Physics and Phenomenology - CP3, Universit{\'e} catholique de Louvain, Louvain-la-Neuve, Belgium \\
$^{44}$ Department of Physics, Mercer University, Macon, GA 31207-0001, USA \\
$^{45}$ Dept. of Astronomy, University of Wisconsin{\textemdash}Madison, Madison, WI 53706, USA \\
$^{46}$ Dept. of Physics and Wisconsin IceCube Particle Astrophysics Center, University of Wisconsin{\textemdash}Madison, Madison, WI 53706, USA \\
$^{47}$ Institute of Physics, University of Mainz, Staudinger Weg 7, D-55099 Mainz, Germany \\
$^{48}$ School of Physics and Astronomy, The University of Manchester, Oxford Road, Manchester, M13 9PL, United Kingdom \\
$^{49}$ Department of Physics, Marquette University, Milwaukee, WI 53201, USA \\
$^{50}$ Dept. of High Energy Physics, Tata Institute of Fundamental Research, Colaba, Mumbai 400 005, India \\
$^{51}$ Institut f{\"u}r Kernphysik, Universit{\"a}t M{\"u}nster, D-48149 M{\"u}nster, Germany \\
$^{52}$ Bartol Research Institute and Dept. of Physics and Astronomy, University of Delaware, Newark, DE 19716, USA \\
$^{53}$ Dept. of Physics, Yale University, New Haven, CT 06520, USA \\
$^{54}$ Columbia Astrophysics and Nevis Laboratories, Columbia University, New York, NY 10027, USA \\
$^{55}$ Dept. of Physics, University of Notre Dame du Lac, 225 Nieuwland Science Hall, Notre Dame, IN 46556-5670, USA \\
$^{56}$ Graduate School of Science and NITEP, Osaka Metropolitan University, Osaka 558-8585, Japan \\
$^{57}$ Dept. of Physics, University of Oxford, Parks Road, Oxford OX1 3PU, United Kingdom \\
$^{58}$ Dipartimento di Fisica e Astronomia Galileo Galilei, Universit{\`a} Degli Studi di Padova, I-35122 Padova PD, Italy \\
$^{59}$ Dept. of Physics, Drexel University, 3141 Chestnut Street, Philadelphia, PA 19104, USA \\
$^{60}$ Physics Department, South Dakota School of Mines and Technology, Rapid City, SD 57701, USA \\
$^{61}$ Dept. of Physics, University of Wisconsin, River Falls, WI 54022, USA \\
$^{62}$ Dept. of Physics and Astronomy, University of Rochester, Rochester, NY 14627, USA \\
$^{63}$ Department of Physics and Astronomy, University of Utah, Salt Lake City, UT 84112, USA \\
$^{64}$ Dept. of Physics, Chung-Ang University, Seoul 06974, Republic of Korea \\
$^{65}$ Oskar Klein Centre and Dept. of Physics, Stockholm University, SE-10691 Stockholm, Sweden \\
$^{66}$ Dept. of Physics and Astronomy, Stony Brook University, Stony Brook, NY 11794-3800, USA \\
$^{67}$ Dept. of Physics, Sungkyunkwan University, Suwon 16419, Republic of Korea \\
$^{68}$ Institute of Basic Science, Sungkyunkwan University, Suwon 16419, Republic of Korea \\
$^{69}$ Institute of Physics, Academia Sinica, Taipei, 11529, Taiwan \\
$^{70}$ Earthquake Research Institute, University of Tokyo, Bunkyo, Tokyo 113-0032, Japan \\
$^{71}$ Dept. of Physics and Astronomy, University of Alabama, Tuscaloosa, AL 35487, USA \\
$^{72}$ Dept. of Astronomy and Astrophysics, Pennsylvania State University, University Park, PA 16802, USA \\
$^{73}$ Dept. of Physics, Pennsylvania State University, University Park, PA 16802, USA \\
$^{74}$ Institute of Gravitation and the Cosmos, Center for Multi-Messenger Astrophysics, Pennsylvania State University, University Park, PA 16802, USA \\
$^{75}$ Dept. of Physics and Astronomy, Uppsala University, Box 516, SE-75120 Uppsala, Sweden \\
$^{76}$ Dept. of Physics, University of Wuppertal, D-42119 Wuppertal, Germany \\
$^{77}$ Deutsches Elektronen-Synchrotron DESY, Platanenallee 6, D-15738 Zeuthen, Germany \\
$^{78}$ Institute of Physics, Sachivalaya Marg, Sainik School Post, Bhubaneswar 751005, India \\
$^{79}$ Department of Space, Earth and Environment, Chalmers University of Technology, 412 96 Gothenburg, Sweden \\
$^{80}$ INFN Padova, I-35131 Padova, Italy \\
$^{81}$ Earthquake Research Institute, University of Tokyo, Bunkyo, Tokyo 113-0032, Japan \\
$^{82}$ INFN Padova, I-35131 Padova, Italy

\subsection*{Acknowledgments}

\noindent
The authors gratefully acknowledge the support from the following agencies and institutions:
USA {\textendash} U.S. National Science Foundation-Office of Polar Programs,
U.S. National Science Foundation-Physics Division,
U.S. National Science Foundation-EPSCoR,
U.S. National Science Foundation-Office of Advanced Cyberinfrastructure,
Wisconsin Alumni Research Foundation,
Center for High Throughput Computing (CHTC) at the University of Wisconsin{\textendash}Madison,
Open Science Grid (OSG),
Partnership to Advance Throughput Computing (PATh),
Advanced Cyberinfrastructure Coordination Ecosystem: Services {\&} Support (ACCESS),
Frontera and Ranch computing project at the Texas Advanced Computing Center,
U.S. Department of Energy-National Energy Research Scientific Computing Center,
Particle astrophysics research computing center at the University of Maryland,
Institute for Cyber-Enabled Research at Michigan State University,
Astroparticle physics computational facility at Marquette University,
NVIDIA Corporation,
and Google Cloud Platform;
Belgium {\textendash} Funds for Scientific Research (FRS-FNRS and FWO),
FWO Odysseus and Big Science programmes,
and Belgian Federal Science Policy Office (Belspo);
Germany {\textendash} Bundesministerium f{\"u}r Bildung und Forschung (BMBF),
Deutsche Forschungsgemeinschaft (DFG),
Helmholtz Alliance for Astroparticle Physics (HAP),
Initiative and Networking Fund of the Helmholtz Association,
Deutsches Elektronen Synchrotron (DESY),
and High Performance Computing cluster of the RWTH Aachen;
Sweden {\textendash} Swedish Research Council,
Swedish Polar Research Secretariat,
Swedish National Infrastructure for Computing (SNIC),
and Knut and Alice Wallenberg Foundation;
European Union {\textendash} EGI Advanced Computing for research;
Australia {\textendash} Australian Research Council;
Canada {\textendash} Natural Sciences and Engineering Research Council of Canada,
Calcul Qu{\'e}bec, Compute Ontario, Canada Foundation for Innovation, WestGrid, and Digital Research Alliance of Canada;
Denmark {\textendash} Villum Fonden, Carlsberg Foundation, and European Commission;
New Zealand {\textendash} Marsden Fund;
Japan {\textendash} Japan Society for Promotion of Science (JSPS)
and Institute for Global Prominent Research (IGPR) of Chiba University;
Korea {\textendash} National Research Foundation of Korea (NRF);
Switzerland {\textendash} Swiss National Science Foundation (SNSF).
